Performance Evaluation of MU-MIMO Under the Impact of Open Loop Traffic Dynamics

Multi-user MIMO enhances throughput by simultaneously transmitting/receiving parallel data streams to/from a group of users. However, the throughput analysis does not ac-count for variable data traffic. The research objective of this project is to analyze the effect of variable traffic as it will change the system behavior. The two characteristic features of variable traffic viz. packet size variation and traffic burstiness have been considered for the analysis in this project. Their effects have been studied individually to provide an insight into the problem. Through simulations, we show that in certain scenarios the system performance of MU-MIMO deteriorates significantly due to both packet size variations and traffic burstiness individually even under ideal conditions with respect to channel variations, channel correlation, mobility, etc. Furthermore, we show that under bursty traffic with higher offered load the aggregate throughput first re-mains steady until a certain peak to average rate ratio and then deteriorates linearly instead of exponentially. Also, un-der high amount of traffic burstiness, the throughputs are in-dependent of the aggregation rates. A thorough analysis is provided to explain these two phenomena. This is the first research work that considers the impact of variable traffic on the performance of MU-MIMO. Therefore, the implications for MAC protocol design are significant.

==> secs/results.tex <==
% !TEX root = ../mypaper.tex
\subsection{Results and Discussion}
\subsubsection{Packet Size Variation}


\emph{{\bf Finding:} To reduce the overhead to data ratio, a MU-MIMO based AP would have to transmit at higher aggregation rates. However, at higher aggregation rates, the drop in throughput would be larger if packet sizes are correlated. However, for uncorrelated packet sizes, this drop is extremely small.}

\subsubsection{Traffic Burstiness}

\emph{{\bf Finding:} Bursty traffic results in aggregation delay and timing alignment issues which have a significant impact on the system performance. Furthermore, this impact increases with increasing aggregation rates and higher aggregation rates are necessary for reducing the overhead to data ratio in MU-MIMO.}

\emph{{\bf Implications for MAC protocol design:} These simulations show that there are certain scenarios with respect to packet size variation and traffic burstiness wherein the performance of a MU-MIMO system begins to deteriorate even under the best possible conditions with respect to channel variations, channel correlation, errors in reception, mobility, etc. The fundamental reason for the degradation in system performance is that data is transmitted simultaneously to multiple users and hence the traffic characteristics of one user affects the others. Therefore, in such situations, the AP should switch to a different transmission scheme such as MISO or SISO depending on which performs better.}

\emph{{\bf Key Challenges:} In order to design such a switching scheme, it is necessary to determine a system level parameter which would fall below or rise above a threshold indicating the need to switch. However, traffic characteristics are largely influenced by the interaction of the user with the server and hence identifying such a parameter might be difficult.}  
